BinSparX: Sparsified Binary Neural Networks for Reduced Hardware Non-Idealities in Xbar Arrays

Compute-in-memory (CiM)-based binary neural network (CiM-BNN) accelerators marry the benefits of CiM and ultra-low precision quantization, making them highly suitable for edge computing. However, CiM-enabled crossbar (Xbar) arrays are plagued with hardware non-idealities like parasitic resistances and device non-linearities that impair inference accuracy, especially in scaled technologies. In this work, we first analyze the impact of Xbar non-idealities on the inference accuracy of various CiM-BNNs, establishing that the unique properties of CiM-BNNs make them more prone to hardware non-idealities compared to higher precision deep neural networks (DNNs). To address this issue, we propose BinSparX, a training-free technique that mitigates non-idealities in CiM-BNNs. BinSparX utilizes the distinct attributes of BNNs to reduce the average current generated during the CiM operations in Xbar arrays. This is achieved by statically and dynamically sparsifying the BNN weights and activations, respectively (which, in the context of BNNs, is defined as reducing the number of +1 weights and activations). This minimizes the IR drops across the parasitic resistances, drastically mitigating their impact on inference accuracy. To evaluate our technique, we conduct experiments on ResNet-18 and VGG-small CiM-BNNs designed at the 7nm technology node using 8T-SRAM and 1T-1ReRAM. Our results show that BinSparX is highly effective in alleviating the impact of non-idealities, recouping the inference accuracy to near-ideal (software) levels in some cases and providing accuracy boost of up to 77.25%. These benefits are accompanied by energy reduction, albeit at the cost of mild latency/area increase.

==> Sections/Acknowledgements.tex <==
\section{Acknowledgements}
\label{sec:acknowledgements}

This work is supported, in part, by the Center for the Co-Design of Cognitive Systems (COCOSYS), one of seven centers in JUMP 2.0, funded by Semiconductor Research Corporation (SRC) and DARPA, and in part, by Raytheon.  
